AnnoCTR: A Dataset for Detecting and Linking Entities, Tactics, and Techniques in Cyber Threat Reports

Monitoring the threat landscape to be aware of actual or potential attacks is of utmost importance to cybersecurity professionals. Information about cyber threats is typically distributed using natural language reports. Natural language processing can help with managing this large amount of unstructured information, yet to date, the topic has received little attention. With this paper, we present AnnoCTR, a new CC-BY-SA-licensed dataset of cyber threat reports. The reports have been annotated by a domain expert with named entities, temporal expressions, and cybersecurity-specific concepts including implicitly mentioned techniques and tactics. Entities and concepts are linked to Wikipedia and the MITRE ATT&CK knowledge base, the most widely-used taxonomy for classifying types of attacks. Prior datasets linking to MITRE ATT&CK either provide a single label per document or annotate sentences out-of-context; our dataset annotates entire documents in a much finer-grained way. In an experimental study, we model the annotations of our dataset using state-of-the-art neural models. In our few-shot scenario, we find that for identifying the MITRE ATT&CK concepts that are mentioned explicitly or implicitly in a text, concept descriptions from MITRE ATT&CK are an effective source for training data augmentation.

==> sections/table_MIMIC3.tex <==
\begin{table*}[]
	\centering
	\small
	\begin{tabular}{@{}l	cc	cc	ccc@{}}
		\toprule
		Method & AUC macro & AUC micro & F1 macro & F1 micro & P@5 & P@8 & P@15 \\
		\midrule
		\rule{0pt}{2.6ex}
		LogisticRegression & 56.1 & 93.7 & 1.1 & 27.2 & - & 54.2 & 41.1 \\
		CAML\cite{mullenbach-etal-2018-explainable} & 89.5 & 98.6 & 8.8 & 53.9 & - & 70.9 & 56.1 \\
		DR-CAML\cite{mullenbach-etal-2018-explainable} & 89.7 & 98.5 & 8.6 & 52.9 & - & 69.0 & 54.8 \\
		MSATT-KG\cite{xie2019ehr} & 91.0 & 99.2 & 9.0 & 55.3 & - & 72.8 & 58.1 \\
		MultiResCNN\cite{li2020icd} & 91.0 & 98.6 & 8.5 & 55.2 & - & 73.4 & 58.4 \\
		LAAT\cite{vu2020label} & 91.9 & 98.8 & 9.9 & 57.5 & 81.3 & 73.8 & 59.1 \\
		JointLAAT\cite{vu2020label} & 92.1 & 98.8 & 10.7 & 57.5 & 80.6 & 73.5 & 59.0 \\
		\midrule
		BERT-ICD\cite{pascual-etal-2021-towards}* & 84.45 & 88.65 &-&-&-&-&-\\
		\bottomrule
	\end{tabular}
	\caption{Results on MIMIC3 dataset, results taken from their papers. *:The BERT-ICD results are in the frequent-50 labels not the full datasets, hence not comparable in this table.}
	\label{tab:results_tram}
\end{table*}
\begin{table*}[]
	\centering
	\small
	\begin{tabular}{@{}l	cc |	cc	|	cc	|	cc@{}}
		\toprule
		Method & fr-R@10 & fr-nDCG@10 & fs-R@10 & fs-nDCG@10 & zs-R@10 & zs-nDCG@10 & R@10 & nDCG@10\\
		\midrule
		CAML & 0.422 & 0.711 & 0.104 & 0.073 & 0.067 & 0.029 & 0.415 & 0.709 \\
		DR-CAML & 0.416 & 0.699 & 0.105 & 0.064 & 0.038 & 0.018 & 0.409 & 0.697 \\
		ZACNN & 0.405 & 0.684 & 0.207 & 0.104 & 0.457 & 0.222 & 0.372 & 0.654 \\
		ZAGCNN & 0.427 & 0.713 & 0.258 & 0.130 & 0.512 & 0.253 & 0.394 & 0.685 \\
		ACNN-KAMG & 0.434 & 0.724 & 0.295 & 0.195 & 0.553 & 0.385 & 0.427 & 0.722 \\
		\bottomrule
	\end{tabular}
	\caption{Results on MIMIC3 dataset, they are taken from \cite{lu-etal-2020-multi}.
	CAML,DR-CAML:\cite{mullenbach-etal-2018-explainable} - ZAXNN,ZAGCNN:\cite{rios-kavuluru-2018-shot} - ACNN-KAMG\cite{lu-etal-2020-multi} }
	\label{tab:results_tram}
\end{table*}



==> sections/table_TRAM_final.tex <==

\begin{table*}[]
	\centering
	\small
	\begin{tabular}{@{}l	cc |	cc	|	cc@{}}
		\toprule
		& \multicolumn{2}{c}{ALL} & \multicolumn{2}{c}{FREQUENT} & \multicolumn{2}{c}{FEW-SHOT}\\
		Method & F1-micro  & F1-weighted & F1-micro  & F1-weighted & F1-micro & F1-weighted \\
		\midrule
		LogisticRegression & 0.51 & 0.44 & 0.814 & 0.816 & 0.148 & 0.203 \\
		CNN1 & 0.468 & 0.413 & 0.713 & 0.715 & 0.176 & 0.227 \\
		CNN1-2phase-1 & 0.414 & 0.357 & 0.636 & 0.634 & 0.148 & 0.204 \\
		CNN1-2phase-2 & 0.418 & 0.363 & 0.651 & 0.649 & 0.139 & 0.197 \\
		CNN1-2phase-3 & 0.384 & 0.317 & 0.636 & 0.631 & 0.083 & 0.131 \\
		VanillaBert & 0.473 & 0.44 & 0.651 & 0.649 & 0.259 & 0.324 \\
		VanillaSciBert1 & 0.57 & 0.541 & 0.736 & 0.75 & 0.37 & 0.432 \\
		VSB-2phase-1 & 0.527 & 0.484 & 0.76 & 0.767 & 0.25 & 0.322 \\
		VSB-2phase-2 & 0.51 & 0.463 & 0.721 & 0.74 & 0.259 & 0.313 \\
		VSB-2phase-3 & 0.46 & 0.428 & 0.62 & 0.611 & 0.269 & 0.35 \\
		VanillaSciBert1Cysec & 0.561 & 0.521 & 0.713 & 0.725 & 0.38 & 0.426 \\
		LWANSciBert1 & 0.553 & 0.517 & 0.729 & 0.744 & 0.343 & 0.412 \\
		BLINK & 0.532 & 0.52 & 0.698 & 0.736 & 0.333 & 0.412 \\ 
		\bottomrule
	\end{tabular}
	\caption{TRAM dataset results on dev split. 24 frequent labels with 129 instances and 75 (31+44) few-shot labels with 108 instances, and 99 total labels with 237 instances.}
	\label{tab:results_tram_dev}
\end{table*}

\begin{table*}[]
	\centering
	\small
	\begin{tabular}{@{}l	cc |	cc	|	cc@{}}
		\toprule
		& \multicolumn{2}{c}{ALL} & \multicolumn{2}{c}{FREQUENT} & \multicolumn{2}{c}{FEW-SHOT}\\
		Method & F1-micro  & F1-weighted & F1-micro  & F1-weighted & F1-micro & F1-weighted \\
		\midrule
		LogisticRegression & 0.47 & 0.398 & 0.711 & 0.702 & 0.136 & 0.183 \\
		CNN1 & 0.431 & 0.379 & 0.639 & 0.646 & 0.143 & 0.181 \\
		VanillaBert & 0.476 & 0.461 & 0.619 & 0.634 & 0.279 & 0.322 \\
		VanillaSciBert1 & 0.548 & 0.52 & 0.701 & 0.717 & \textbf{0.336} & 0.374 \\
		VanillaSciBert1Cysec & 0.545 & 0.517 & 0.701 & 0.713 & 0.329 & 0.389 \\
		LWANSciBert1 & 0.554 & 0.522 & 0.722 & 0.724 & 0.321 & 0.377 \\
		BLINK & 0.497 & 0.482 & 0.624 & 0.642 & 0.321 & \textbf{0.394} \\ 
		\bottomrule
	\end{tabular}
	\caption{TRAM dataset results on test split. 24 frequent labels with 194 instances and 75 (31+44) few-shot labels with 140 instances, and 99(55+44) total labels with 334 instances.}
	\label{tab:results_tram_test}
\end{table*}

==> sections/table_USPTO.tex <==
\begin{table*}[]
	\centering
	\small
	\begin{tabular}{@{}l	cc |	cc	|	cc@{}}
		\toprule
		Method & R@10 & nDCG@10 & fr-R@10 & fr-nDCG@10 & fs-R@10 & fs-nDCG@10 \\
		\midrule
		FLAT-CLS & 0.812 &  0.754 & 0.812 & 0.754 & 0.472 & 0.429\\
		TMM-CLS & 0.843 & 0.782 & 0.843 & 0.782 & 0.555 & 0.504\\
		THMM-CLS &  &  &  &  &  &  \\
		\bottomrule
	\end{tabular}
	\caption{Results on USPTO dataset few-shot-threshold=10, all (10000), fr=frequent (9995), fs=few-shot (136).\\
	NOTE:these are all the "leaf" label evaluation only.}
	\label{tab:results_uspto}
\end{table*}
\begin{table*}[]
	\centering
	\small	
	\begin{tabular}{@{}l	cc |	cc	|	cc@{}}
		\toprule
		Method & R@10 & nDCG@10 & fr-R@10 & fr-nDCG@10 & fs-R@10 & fs-nDCG@10 \\
		\midrule
		FLAT-CLS & 0.812 & 0.754 & 0.813 & 0.755 & 0.488 & 0.443\\
		TMM-CLS & 0.843 & 0.782 & 0.843 & 0.783 & 0.558 & 0.509\\
		THMM-CLS &  &  &  &  &  &  \\
		\bottomrule
	\end{tabular}
	\caption{Results on USPTO dataset few-shot-threshold=15, all (10000), fr=frequent (9978), fs=few-shot (264)).\\
		NOTE:these are all the "leaf" label evaluation only.}
	\label{tab:results_uspto}
\end{table*}

